Reach-avoid games for players with damped double integrator dynamics

This paper investigates a reach-avoid game between two players with damped double integrator dynamics. An optimal state-feedback strategy is derived using a differential game framework combined with geometric analysis. To facilitate the analysis, we introduce the concept of multiple reachable region by characterizing the motion of players with damped double integrator dynamics. Based on this, a new type of the attackers dominance region is introduced. We show that distinct strategies are required depending on the location of the terminal position within different areas of the attacker's dominance region. Furthermore, we prove that the proposed strategies satisfy the necessary condition for optimality. Numerical simulations are provided to illustrate the conclusions.

==> fig/example1/dAD.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.9290, 0.6940, 0.1250}%
\definecolor{mycolor3}{rgb}{0.20000,0.30000,0.70000}%
\definecolor{mycolor4}{rgb}{0.86000,0.08000,0.24000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=6.521cm,
height=3.566cm,
at={(0,0)},
scale only axis,
xlabel={$t$},
xlabel style={
    font=\color{white!15!black},
    at={(axis description cs:1.1,0.05)}, % 右下角（底部右端）
    anchor=north east
},
tick label style={font=\tiny},
xmin=0,
xmax=3,
ymin=0,
ymax=5.5,
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black,font=\tiny}
]
\addplot [color=mycolor2]
  table[row sep=crcr]{%
0.0250000000000002	5.04507568177755\\
0.0500000000000009	4.99110665278345\\
0.0749999999999999	4.9371104450084\\
0.0999999999999971	4.88308524306566\\
0.124999999999994	4.82902938836769\\
0.149999999999992	4.77494137019074\\
0.174999999999989	4.72081981719594\\
0.199999999999986	4.66666348923312\\
0.224999999999983	4.61247126999705\\
0.249999999999981	4.55824215950986\\
0.274999999999978	4.50397526724856\\
0.299999999999975	4.44966980583113\\
0.324999999999972	4.39532508446836\\
0.34999999999997	4.34094050330967\\
0.374999999999967	4.28651554779007\\
0.399999999999964	4.23204978327698\\
0.424999999999961	4.1775428501996\\
0.449999999999959	4.12299445905689\\
0.474999999999956	4.06840438631485\\
0.499999999999953	4.01377246948828\\
0.52499999999995	3.95909860352395\\
0.549999999999948	3.90438273693144\\
0.574999999999945	3.84962486816371\\
0.599999999999942	3.79482504217507\\
0.624999999999939	3.73998334706443\\
0.649999999999937	3.68509991115953\\
0.674999999999934	3.6301748998368\\
0.699999999999931	3.57520851306416\\
0.724999999999928	3.52020098261928\\
0.749999999999926	3.46515256984216\\
0.774999999999923	3.41006356311241\\
0.79999999999992	3.3549342758221\\
0.824999999999917	3.29976504413611\\
0.849999999999915	3.24455622513913\\
0.874999999999912	3.18930819496795\\
0.899999999999909	3.13402134714333\\
0.924999999999906	3.07869609105062\\
0.949999999999904	3.02333285015726\\
0.974999999999901	2.9679320607472\\
0.999999999999898	2.91249417051734\\
1.02499999999995	2.8570196369418\\
1.05	2.80150892649288\\
1.07500000000006	2.74596251358051\\
1.10000000000011	2.69038087937717\\
1.12500000000016	2.63476451121619\\
1.15000000000021	2.57911390026814\\
1.17500000000027	2.52342954211347\\
1.20000000000032	2.46771193563731\\
1.22500000000037	2.41196158155669\\
1.25000000000043	2.35617898246027\\
1.27500000000048	2.30036464241733\\
1.30000000000053	2.244519065086\\
1.32500000000058	2.18864275380758\\
1.35000000000064	2.13273621152102\\
1.37500000000069	2.07679994051507\\
1.40000000000074	2.02083444018066\\
1.42500000000079	1.96484020826208\\
1.45000000000085	1.90881773977429\\
1.4750000000009	1.85276752694691\\
1.50000000000095	1.79669005920743\\
1.52500000000101	1.7405858212693\\
1.55000000000106	1.6844552943627\\
1.57500000000111	1.62829895561387\\
1.60000000000116	1.57211727837473\\
1.62500000000122	1.51591073067591\\
1.65000000000127	1.45967977607892\\
1.67500000000132	1.40342487338742\\
1.70000000000138	1.34714647601236\\
1.72500000000143	1.29084503185909\\
1.75000000000148	1.23452098396536\\
1.77500000000153	1.17817476901194\\
1.80000000000159	1.1218068193052\\
1.82500000000164	1.06541756099965\\
1.85000000000169	1.00900741319931\\
1.87500000000174	0.952576790090229\\
1.9000000000018	0.89612609969473\\
1.92500000000185	0.839655744201556\\
1.9500000000019	0.783166120490201\\
1.97500000000196	0.726657619282951\\
2.00000000000201	0.67013062440134\\
2.02500000000195	0.613585513887669\\
2.05000000000189	0.557022659326394\\
2.07500000000183	0.500442428618008\\
2.10000000000178	0.443845180191848\\
2.12500000000172	0.387231282661096\\
2.15000000000166	0.330601069208404\\
2.1750000000016	0.273954918303344\\
2.20000000000154	0.217293153621584\\
2.22500000000148	0.160616315530382\\
2.25000000000143	0.10392536057037\\
2.27500000000137	0.0472244638123898\\
};
\addlegendentry{($\theta_D^*$,$\theta_A^*$)}

\addplot [color=mycolor3]
  table[row sep=crcr]{%
0.0250000000000002	5.04496312718834\\
0.0500000000000009	4.99066215180836\\
0.0749999999999999	4.93612290904779\\
0.0999999999999971	4.88135153456422\\
0.124999999999994	4.82635398331877\\
0.149999999999992	4.77113603448422\\
0.174999999999989	4.71570329623476\\
0.199999999999986	4.66006121034219\\
0.224999999999983	4.6042150565492\\
0.249999999999981	4.54816995679499\\
0.274999999999978	4.49193087928234\\
0.299999999999975	4.43550264238298\\
0.324999999999972	4.37888991835855\\
0.34999999999997	4.32209723699375\\
0.374999999999967	4.26512898904768\\
0.399999999999964	4.20798942959741\\
0.424999999999961	4.15068268127021\\
0.449999999999959	4.09321273725036\\
0.474999999999956	4.03558346430367\\
0.499999999999953	3.97779860563757\\
0.52499999999995	3.91986178364352\\
0.549999999999948	3.86177650252527\\
0.574999999999945	3.80354615085574\\
0.599999999999942	3.74517400400591\\
0.624999999999939	3.6866632265063\\
0.649999999999937	3.62801687427733\\
0.674999999999934	3.56923789681412\\
0.699999999999931	3.51032913928174\\
0.724999999999928	3.45129334447172\\
0.749999999999926	3.39213315474904\\
0.774999999999923	3.33285111385728\\
0.79999999999992	3.27344966868742\\
0.824999999999917	3.21393117094576\\
0.849999999999915	3.15429787875926\\
0.874999999999912	3.0945519582153\\
0.899999999999909	3.03469548477754\\
0.924999999999906	2.97473044468999\\
0.949999999999904	2.9146587362891\\
0.974999999999901	2.85448217123688\\
0.999999999999898	2.79420247571066\\
1.02499999999995	2.73382129148587\\
1.05	2.6733401769948\\
1.07500000000006	2.61276060827857\\
1.10000000000011	2.55208397988613\\
1.12500000000016	2.49131160573388\\
1.15000000000021	2.43044471987291\\
1.17500000000027	2.3694844772005\\
1.20000000000032	2.30843195406387\\
1.22500000000037	2.24728814887683\\
1.25000000000043	2.18605398263057\\
1.27500000000048	2.12473029931809\\
1.30000000000053	2.06331786636076\\
1.32500000000058	2.00181737490696\\
1.35000000000064	1.94022944012981\\
1.37500000000069	1.87855460137478\\
1.40000000000074	1.81679332242242\\
1.42500000000079	1.75494599137284\\
1.45000000000085	1.69301292087591\\
1.4750000000009	1.6309943479831\\
1.50000000000095	1.56889043578449\\
1.52500000000101	1.50670127027214\\
1.55000000000106	1.44442686048432\\
1.57500000000111	1.38206714147121\\
1.60000000000116	1.31962197256941\\
1.62500000000122	1.25709113772705\\
1.65000000000127	1.19447434577682\\
1.67500000000132	1.13177123101898\\
1.70000000000138	1.06898135421753\\
1.72500000000143	1.00610420406076\\
1.75000000000148	0.943139199538943\\
1.77500000000153	0.880085693436001\\
1.80000000000159	0.816942977283279\\
1.82500000000164	0.753710289505987\\
1.85000000000169	0.690386826585665\\
1.87500000000174	0.62697175983622\\
1.9000000000018	0.563464261986487\\
1.92500000000185	0.499863546115503\\
1.9500000000019	0.436168928122734\\
1.97500000000196	0.372379928037975\\
2.00000000000201	0.308496443088501\\
2.02500000000195	0.244519061100844\\
2.05000000000189	0.180464864218386\\
2.07500000000183	0.117777749624149\\
2.10000000000178	0.05738068987146\\
};
\addlegendentry{($\theta_D^*$,pure-pursuit)}

\addplot [color=mycolor4]
  table[row sep=crcr]{%
0.0250000000000002	5.04505039543969\\
0.0500000000000009	4.99100470279738\\
0.0749999999999999	4.936879420923\\
0.0999999999999971	4.88267192695378\\
0.124999999999994	4.82837997406069\\
0.149999999999992	4.77400167670484\\
0.174999999999989	4.71953549618302\\
0.199999999999986	4.66498022725864\\
0.224999999999983	4.61033498597375\\
0.249999999999981	4.55559919782433\\
0.274999999999978	4.50077258683797\\
0.299999999999975	4.44585516536202\\
0.324999999999972	4.39084722484751\\
0.34999999999997	4.33574932706071\\
0.374999999999967	4.28056229621905\\
0.399999999999964	4.22528721194124\\
0.424999999999961	4.1699254027072\\
0.449999999999959	4.11447844020949\\
0.474999999999956	4.0589481343921\\
0.499999999999953	4.00333652886481\\
0.52499999999995	3.94764589844864\\
0.549999999999948	3.89187874575006\\
0.574999999999945	3.83603779910595\\
0.599999999999942	3.7801260114882\\
0.624999999999939	3.72414655999328\\
0.649999999999937	3.66810284628899\\
0.674999999999934	3.61199849777699\\
0.699999999999931	3.55583736928081\\
0.724999999999928	3.49962354615966\\
0.749999999999926	3.44336134780434\\
0.774999999999923	3.38705533205015\\
0.79999999999992	3.33071030048876\\
0.824999999999917	3.2743313040557\\
0.849999999999915	3.21792365272368\\
0.874999999999912	3.16149292101173\\
0.899999999999909	3.10504495776826\\
0.924999999999906	3.04858589596925\\
0.949999999999904	2.99212216390812\\
0.974999999999901	2.9356604956997\\
0.999999999999898	2.87920794415126\\
1.02499999999995	2.8227718927869\\
1.05	2.76636006883485\\
1.07500000000006	2.70998055546898\\
1.10000000000011	2.65364180431504\\
1.12500000000016	2.59735264529142\\
1.15000000000021	2.54112229672729\\
1.17500000000027	2.48496036923703\\
1.20000000000032	2.42887686641642\\
1.22500000000037	2.37288217803814\\
1.25000000000043	2.31698706343154\\
1.27500000000048	2.26120262140972\\
1.30000000000053	2.20554024189537\\
1.32500000000058	2.15001153402369\\
1.35000000000064	2.09462822291769\\
1.37500000000069	2.03940200874874\\
1.40000000000074	1.98434438192363\\
1.42500000000079	1.92946639122474\\
1.45000000000085	1.87477837841061\\
1.4750000000009	1.82028971528583\\
1.50000000000095	1.76600863747702\\
1.52500000000101	1.7119423375926\\
1.55000000000106	1.65809756604615\\
1.57500000000111	1.60448195919374\\
1.60000000000116	1.55110608019577\\
1.62500000000122	1.4979857601029\\
1.65000000000127	1.44514413544096\\
1.67500000000132	1.39261300449593\\
1.70000000000138	1.34043361013702\\
1.72500000000143	1.28865718232367\\
1.75000000000148	1.23734550200795\\
1.77500000000153	1.18657177299387\\
1.80000000000159	1.13642174766775\\
1.82500000000164	1.08699525178868\\
1.85000000000169	1.03840808434198\\
1.87500000000174	0.990794298459583\\
1.9000000000018	0.94430883451348\\
1.92500000000185	0.899130446793396\\
1.9500000000019	0.855464778679353\\
1.97500000000196	0.813547324897714\\
2.00000000000201	0.773645831601137\\
2.02500000000195	0.736061421723753\\
2.05000000000189	0.701127411591392\\
2.07500000000183	0.669204442538679\\
2.10000000000178	0.640670334181683\\
2.12500000000172	0.615903205755185\\
2.15000000000166	0.595257224011235\\
2.1750000000016	0.579032053453702\\
2.20000000000154	0.567439583197715\\
2.22500000000148	0.560573983271014\\
2.25000000000143	0.558392220286097\\
2.27500000000137	0.560710650258106\\
2.30000000000131	0.567219243727799\\
2.32500000000125	0.577510078777522\\
2.35000000000119	0.591113288974024\\
2.37500000000113	0.607533030073516\\
2.40000000000108	0.626277875255483\\
2.42500000000102	0.646882924567878\\
2.45000000000096	0.668923451546149\\
2.4750000000009	0.692021449836651\\
2.50000000000084	0.715847006791088\\
2.52500000000078	0.740116350267865\\
2.55000000000073	0.764588039240932\\
2.57500000000067	0.789058334966208\\
2.60000000000061	0.813356414417965\\
2.62500000000055	0.837339807861341\\
2.65000000000049	0.86089025254427\\
2.67500000000044	0.883910035931228\\
2.70000000000038	0.906318832599774\\
2.72500000000032	0.928051002550223\\
2.75000000000026	0.949053302141032\\
2.7750000000002	0.969282954331495\\
2.80000000000014	0.988706026058016\\
2.82500000000009	1.00729606547096\\
2.85000000000003	1.0250329574497\\
2.87499999999997	1.04190196095685\\
2.89999999999991	1.05789289881928\\
2.92499999999985	1.07299947474379\\
2.94999999999979	1.08721869544346\\
2.97499999999974	1.10055038111543\\
2.99999999999968	1.11299674975777\\
3.02499999999962	1.12456206320289\\
3.04999999999956	1.13525232484983\\
3.0749999999995	1.14507502134034\\
3.09999999999944	1.15403890074777\\
3.12499999999939	1.16215378225916\\
3.14999999999933	1.16943039192195\\
3.17499999999927	1.17588022122481\\
3.19999999999921	1.18151540488975\\
3.22499999999915	1.18634861512546\\
3.24999999999909	1.19039296964504\\
3.27499999999904	1.1936619523556\\
3.29999999999898	1.19616934428855\\
3.32499999999892	1.19792916371736\\
3.34999999999886	1.19895561412318\\
3.3749999999988	1.1992639455213\\
3.39999999999875	1.19887652637707\\
3.42499999999869	1.19780968054641\\
3.44999999999863	1.19607860585338\\
3.47499999999857	1.19369840788896\\
3.49999999999851	1.19068426915525\\
3.52499999999845	1.18705096807118\\
3.5499999999984	1.18281335693849\\
3.57499999999834	1.17798616207167\\
3.59999999999828	1.17258408198883\\
3.62499999999822	1.16662159009162\\
3.64999999999816	1.16011308034849\\
3.6749999999981	1.15307286914586\\
3.69999999999805	1.14551451565744\\
3.72499999999799	1.13745255707469\\
3.74999999999793	1.12890085797079\\
3.77499999999787	1.11987321200847\\
3.79999999999781	1.11038321420297\\
3.82499999999775	1.10044451243822\\
3.8499999999977	1.09007035294507\\
3.87499999999764	1.07927380706527\\
3.89999999999758	1.06806796643277\\
3.92499999999752	1.05646590656284\\
3.94999999999746	1.04448067019657\\
3.97499999999741	1.03212504681648\\
3.99999999999735	1.01941171721483\\
4.02499999999729	1.00635341183638\\
4.04999999999723	0.992962693494783\\
4.07499999999717	0.97925209810277\\
4.09999999999711	0.965234072176046\\
4.12499999999706	0.950921084642208\\
4.149999999997	0.936325695234538\\
4.17499999999694	0.921461007712498\\
4.19999999999688	0.906338036727391\\
4.22499999999682	0.890968857812034\\
4.24999999999676	0.875344068218231\\
4.27499999999671	0.85937001041503\\
4.29999999999665	0.843045513781683\\
4.32499999999659	0.826386596491863\\
4.34999999999653	0.809409645892851\\
4.37499999999647	0.792131457478836\\
4.39999999999641	0.774569275925631\\
4.42499999999636	0.756740851043857\\
4.4499999999963	0.73866449652003\\
4.47499999999624	0.720359152717205\\
4.49999999999618	0.70184446082308\\
4.52499999999612	0.683140841683078\\
4.54999999999607	0.66426959842351\\
4.57499999999601	0.645253025942582\\
4.59999999999595	0.626114528414005\\
4.62499999999589	0.606878752172477\\
4.64999999999583	0.587571743076378\\
4.67499999999577	0.568221133496118\\
4.69999999999572	0.548856331352335\\
4.72499999999566	0.529508785410737\\
4.7499999999956	0.510212147455378\\
4.77499999999554	0.491002553862112\\
4.79999999999548	0.471918962054092\\
4.82499999999542	0.453003461532056\\
4.84999999999537	0.43430159765899\\
4.87499999999531	0.41586275633199\\
4.89999999999525	0.397740474559484\\
4.92499999999519	0.379992748915483\\
4.94999999999513	0.362682293400861\\
4.97499999999507	0.345876585627292\\
4.99999999999502	0.329647799402085\\
5.02499999999496	0.314072304326185\\
5.0499999999949	0.299229796854609\\
5.07499999999484	0.285201811056627\\
5.09999999999478	0.272069694852725\\
5.12499999999473	0.259911085930586\\
5.14999999999467	0.248795562370483\\
5.17499999999461	0.238779506571449\\
5.19999999999455	0.229900417244641\\
5.22499999999449	0.222171265823107\\
5.24999999999443	0.215575716857099\\
5.27499999999438	0.210065105938673\\
5.29999999999432	0.205557902139465\\
5.32499999999426	0.201941955001773\\
5.3499999999942	0.198930411278197\\
};
\addlegendentry{(pure-pursuit,$\theta_A^*$)}
\end{axis}
\end{tikzpicture}%

==> fig/example1/dtarget.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.9290, 0.6940, 0.1250}%
\definecolor{mycolor3}{rgb}{0.20000,0.30000,0.70000}%
\definecolor{mycolor4}{rgb}{0.86000,0.08000,0.24000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=6.521cm,
height=3.566cm,
at={(0,0)},
scale only axis,
xlabel={$t$},
xlabel style={
    font=\color{white!15!black},
    at={(axis description cs:1.1,0.05)}, % 右下角（底部右端）
    anchor=north east
},
tick label style={font=\tiny},
xmin=0,
xmax=3,
ymin=2.5,
ymax=3.8,
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black,font=\tiny}
]
\addplot [color=mycolor2]
  table[row sep=crcr]{%
0.0250000000000002	3.61902352985592\\
0.0500000000000009	3.63171090587441\\
0.0749999999999999	3.64362234110203\\
0.0999999999999971	3.65476737147129\\
0.124999999999994	3.66515604738393\\
0.149999999999992	3.67479885832461\\
0.174999999999989	3.68370666511767\\
0.199999999999986	3.69189063900993\\
0.224999999999983	3.69936220710882\\
0.249999999999981	3.70613300319878\\
0.274999999999978	3.71221482369086\\
0.299999999999975	3.71761958818156\\
0.324999999999972	3.72235930390817\\
0.34999999999997	3.72644603410215\\
0.374999999999967	3.72989186957547\\
0.399999999999964	3.73270890332836\\
0.424999999999961	3.73490920795333\\
0.449999999999959	3.7365048153761\\
0.474999999999956	3.73750769903929\\
0.499999999999953	3.73792975775581\\
0.52499999999995	3.73778280174417\\
0.549999999999948	3.73707854016097\\
0.574999999999945	3.73582857014501\\
0.599999999999942	3.73404436721092\\
0.624999999999939	3.73173727683868\\
0.649999999999937	3.72891850725897\\
0.674999999999934	3.72559912310828\\
0.699999999999931	3.72179004017382\\
0.724999999999928	3.71750202081344\\
0.749999999999926	3.71274567024497\\
0.774999999999923	3.70753143338316\\
0.79999999999992	3.70186959240224\\
0.824999999999917	3.69577026474752\\
0.849999999999915	3.68924340173046\\
0.874999999999912	3.68229878753619\\
0.899999999999909	3.67494603866733\\
0.924999999999906	3.66719460376965\\
0.949999999999904	3.65905376367989\\
0.974999999999901	3.65053263190126\\
0.999999999999898	3.64164015527857\\
1.02499999999995	3.63238511481899\\
1.05	3.62277612696357\\
1.07500000000006	3.61282164494315\\
1.10000000000011	3.60252996025045\\
1.12500000000016	3.59190920441745\\
1.15000000000021	3.58096735039215\\
1.17500000000027	3.56971221488735\\
1.20000000000032	3.55815146031342\\
1.22500000000037	3.54629259667754\\
1.25000000000043	3.534142984002\\
1.27500000000048	3.52170983466854\\
1.30000000000053	3.509000215359\\
1.32500000000058	3.49602104962972\\
1.35000000000064	3.48277912046297\\
1.37500000000069	3.46928107279439\\
1.40000000000074	3.45553341545691\\
1.42500000000079	3.44154252418898\\
1.45000000000085	3.42731464394922\\
1.4750000000009	3.4128558915434\\
1.50000000000095	3.39817225826387\\
1.52500000000101	3.383269611951\\
1.55000000000106	3.36815369999797\\
1.57500000000111	3.35283015178689\\
1.60000000000116	3.33730448140094\\
1.62500000000122	3.32158208975144\\
1.65000000000127	3.30566826741906\\
1.67500000000132	3.28956819713104\\
1.70000000000138	3.27328695611252\\
1.72500000000143	3.25682951857683\\
1.75000000000148	3.24020075842809\\
1.77500000000153	3.22340545128485\\
1.80000000000159	3.20644827755742\\
1.82500000000164	3.18933382433512\\
1.85000000000169	3.17206658751987\\
1.87500000000174	3.15465097488672\\
1.9000000000018	3.13709130806589\\
1.92500000000185	3.11939182499615\\
1.9500000000019	3.10155668242311\\
1.97500000000196	3.08358995792796\\
2.00000000000201	3.06549565197406\\
2.02500000000195	3.04727769052705\\
2.05000000000189	3.02893992709178\\
2.07500000000183	3.01048614582195\\
2.10000000000178	2.99192006183313\\
2.12500000000172	2.9732453298868\\
2.15000000000166	2.95446553157356\\
2.1750000000016	2.9355842040861\\
2.20000000000154	2.91660480949294\\
2.22500000000148	2.89753082825903\\
2.25000000000143	2.87836583409504\\
2.27500000000137	2.85911445262873\\
};
\addlegendentry{($\theta_D^*$,$\theta_A^*$)}

\addplot [color=mycolor3]
  table[row sep=crcr]{%
0.0250000000000002	3.61899526580643\\
0.0500000000000009	3.63160158527412\\
0.0749999999999999	3.64338437583439\\
0.0999999999999971	3.65435788448977\\
0.124999999999994	3.66453642417864\\
0.149999999999992	3.67393433896481\\
0.174999999999989	3.6825659730745\\
0.199999999999986	3.69044564338672\\
0.224999999999983	3.6975876150257\\
0.249999999999981	3.70400607974123\\
0.274999999999978	3.7097151367961\\
0.299999999999975	3.71472877610921\\
0.324999999999972	3.71906086342912\\
0.34999999999997	3.72272512733599\\
0.374999999999967	3.72573514789054\\
0.399999999999964	3.72810434676709\\
0.424999999999961	3.72984597872421\\
0.449999999999959	3.73097312428095\\
0.474999999999956	3.73149868348005\\
0.499999999999953	3.73143537063089\\
0.52499999999995	3.73079570993552\\
0.549999999999948	3.72959203191081\\
0.574999999999945	3.72783647052757\\
0.599999999999942	3.72554096099561\\
0.624999999999939	3.72271723813021\\
0.649999999999937	3.71937683524165\\
0.674999999999934	3.71553108349496\\
0.699999999999931	3.71119111169203\\
0.724999999999928	3.7063678464325\\
0.749999999999926	3.70107201261431\\
0.774999999999923	3.6953141342379\\
0.79999999999992	3.68910453548179\\
0.824999999999917	3.68245334201991\\
0.849999999999915	3.67537048255409\\
0.874999999999912	3.66786569053723\\
0.899999999999909	3.65994850606514\\
0.924999999999906	3.65162827791687\\
0.949999999999904	3.64291416572533\\
0.974999999999901	3.63381514226162\\
0.999999999999898	3.62433999581785\\
1.02499999999995	3.61449733267486\\
1.05	3.60429557964227\\
1.07500000000006	3.59374298665963\\
1.10000000000011	3.58284762944821\\
1.12500000000016	3.5716174122043\\
1.15000000000021	3.56006007032532\\
1.17500000000027	3.54818317316123\\
1.20000000000032	3.53599412678406\\
1.22500000000037	3.52350017676945\\
1.25000000000043	3.51070841098431\\
1.27500000000048	3.49762576237554\\
1.30000000000053	3.48425901175503\\
1.32500000000058	3.47061479057681\\
1.35000000000064	3.45669958370257\\
1.37500000000069	3.44251973215202\\
1.40000000000074	3.4280814358352\\
1.42500000000079	3.41339075626378\\
1.45000000000085	3.39845361923921\\
1.4750000000009	3.38327581751519\\
1.50000000000095	3.36786301343284\\
1.52500000000101	3.35222074152668\\
1.55000000000106	3.33635441109995\\
1.57500000000111	3.32026930876808\\
1.60000000000116	3.30397060096898\\
1.62500000000122	3.28746333643934\\
1.65000000000127	3.27075244865603\\
1.67500000000132	3.25384275824186\\
1.70000000000138	3.23673897533526\\
1.72500000000143	3.21944570192323\\
1.75000000000148	3.20196743413732\\
1.77500000000153	3.18430856451229\\
1.80000000000159	3.16647338420734\\
1.82500000000164	3.14846608518964\\
1.85000000000169	3.13029076238029\\
1.87500000000174	3.11195141576258\\
1.9000000000018	3.0934519524527\\
1.92500000000185	3.07479618873299\\
1.9500000000019	3.05598785204794\\
1.97500000000196	3.03703058296303\\
2.00000000000201	3.01792793708685\\
2.02500000000195	2.9986833869566\\
2.05000000000189	2.97930032388743\\
2.07500000000183	2.95978205978584\\
2.10000000000178	2.94013182892757\\
};
\addlegendentry{($\theta_D^*$,pure-pursuit)}

\addplot [color=mycolor4]
  table[row sep=crcr]{%
0.0250000000000002	3.61902355916593\\
0.0500000000000009	3.63171113908647\\
0.0749999999999999	3.64362312370247\\
0.0999999999999971	3.65476921615635\\
0.124999999999994	3.66515963118376\\
0.149999999999992	3.67480502059002\\
0.174999999999989	3.68371640608787\\
0.199999999999986	3.69190511909417\\
0.224999999999983	3.69938274684498\\
0.249999999999981	3.70616108388124\\
0.274999999999978	3.7122520885946\\
0.299999999999975	3.71766784426682\\
0.324999999999972	3.72242052428416\\
0.34999999999997	3.72652236089983\\
0.374999999999967	3.72998561739775\\
0.399999999999964	3.73282256329183\\
0.424999999999961	3.73504545215149\\
0.449999999999959	3.73666650194869\\
0.474999999999956	3.73769787760911\\
0.499999999999953	3.73815167543091\\
0.52499999999995	3.73803990987587\\
0.549999999999948	3.73737450131827\\
0.574999999999945	3.73616726553002\\
0.599999999999942	3.73442990458534\\
0.624999999999939	3.73217399890015\\
0.649999999999937	3.72941100042797\\
0.674999999999934	3.72615222679802\\
0.699999999999931	3.72240885621212\\
0.724999999999928	3.71819192334922\\
0.749999999999926	3.71351231576689\\
0.774999999999923	3.70838077091493\\
0.79999999999992	3.70280787365988\\
0.824999999999917	3.69680405398195\\
0.849999999999915	3.69037958626325\\
0.874999999999912	3.68354458679713\\
0.899999999999909	3.67630901276846\\
0.924999999999906	3.66868266091547\\
0.949999999999904	3.66067516631275\\
0.974999999999901	3.65229600033283\\
0.999999999999898	3.64355446887876\\
1.02499999999995	3.63445970946697\\
1.05	3.62502068773336\\
1.07500000000006	3.61524619251025\\
1.10000000000011	3.60514482969498\\
1.12500000000016	3.59472501352279\\
1.15000000000021	3.58399495621451\\
1.17500000000027	3.57296265311321\\
1.20000000000032	3.56163586431485\\
1.22500000000037	3.55002209080611\\
1.25000000000043	3.53812854399391\\
1.27500000000048	3.52596210709629\\
1.30000000000053	3.51352928662099\\
1.32500000000058	3.50083615246735\\
1.35000000000064	3.487888264965\\
1.37500000000069	3.47469058911359\\
1.40000000000074	3.46124739861513\\
1.42500000000079	3.44756217682973\\
1.45000000000085	3.43363753269771\\
1.4750000000009	3.41947516245396\\
1.50000000000095	3.40507590895008\\
1.52500000000101	3.39043997944383\\
1.55000000000106	3.37556736643591\\
1.57500000000111	3.36045842948705\\
1.60000000000116	3.34511446417724\\
1.62500000000122	3.32953802200973\\
1.65000000000127	3.31373286872472\\
1.67500000000132	3.29770367936369\\
1.70000000000138	3.28145566583626\\
1.72500000000143	3.26499426930208\\
1.75000000000148	3.24832495594019\\
1.77500000000153	3.23145309600996\\
1.80000000000159	3.2143839048912\\
1.82500000000164	3.19712241697795\\
1.85000000000169	3.17967347924955\\
1.87500000000174	3.16204175498358\\
1.9000000000018	3.14423173286972\\
1.92500000000185	3.12624773813591\\
1.9500000000019	3.10809394454765\\
1.97500000000196	3.0897743863311\\
2.00000000000201	3.07129296961552\\
2.02500000000195	3.05265348340965\\
2.05000000000189	3.03385960982824\\
2.07500000000183	3.01491493360918\\
2.10000000000178	2.99582295084667\\
2.12500000000172	2.97658707683461\\
2.15000000000166	2.95721065283439\\
2.1750000000016	2.93769695177138\\
2.20000000000154	2.91804918274771\\
2.22500000000148	2.89827049421761\\
2.25000000000143	2.87836397603415\\
2.27500000000137	2.85833266044774\\
2.30000000000131	2.83817952229979\\
2.32500000000125	2.81790747871126\\
2.35000000000119	2.79751938852253\\
2.37500000000113	2.77701805171473\\
2.40000000000108	2.75640620895163\\
2.42500000000102	2.73568654136672\\
2.45000000000096	2.71486167057461\\
2.4750000000009	2.69393415892745\\
2.50000000000084	2.67290650998898\\
2.52500000000078	2.6517811691849\\
2.55000000000073	2.63056052460194\\
2.57500000000067	2.60924690788163\\
2.60000000000061	2.58784259520133\\
2.62500000000055	2.566349808316\\
2.65000000000049	2.54477071562576\\
2.67500000000044	2.52310743327809\\
2.70000000000038	2.50136202627899\\
2.72500000000032	2.47953650960869\\
2.75000000000026	2.45763284933114\\
2.7750000000002	2.43565296370284\\
2.80000000000014	2.41359872426567\\
2.82500000000009	2.39147195692889\\
2.85000000000003	2.3692744430405\\
2.87499999999997	2.3470079204194\\
2.89999999999991	2.32467408438455\\
2.92499999999985	2.30227458877985\\
2.94999999999979	2.27981104695646\\
2.97499999999974	2.25728503274149\\
2.99999999999968	2.23469808138994\\
3.02499999999962	2.21205169051495\\
3.04999999999956	2.18934732099364\\
3.0749999999995	2.16658639786196\\
3.09999999999944	2.14377031118068\\
3.12499999999939	2.12090041689083\\
3.14999999999933	2.09797803763971\\
3.17499999999927	2.07500446359663\\
3.19999999999921	2.05198095324949\\
3.22499999999915	2.02890873418312\\
3.24999999999909	2.00578900383211\\
3.27499999999904	1.98262293022774\\
3.29999999999898	1.95941165272213\\
3.32499999999892	1.9361562826979\\
3.34999999999886	1.9128579042607\\
3.3749999999988	1.88951890044591\\
3.39999999999875	1.86615173951694\\
3.42499999999869	1.84275972046867\\
3.44999999999863	1.81934443270829\\
3.47499999999857	1.7959073619043\\
3.49999999999851	1.77245012019148\\
3.52499999999845	1.74897389804262\\
3.5499999999984	1.72548004111389\\
3.57499999999834	1.70196984118228\\
3.59999999999828	1.67844465168376\\
3.62499999999822	1.65490568344078\\
3.64999999999816	1.63135416249548\\
3.6749999999981	1.60779133435613\\
3.69999999999805	1.58421784415146\\
3.72499999999799	1.56063529576569\\
3.74999999999793	1.53704479255749\\
3.77499999999787	1.5134474511264\\
3.79999999999781	1.48984430168629\\
3.82499999999775	1.46623646629104\\
3.8499999999977	1.44262483730022\\
3.87499999999764	1.41901022462321\\
3.89999999999758	1.39539348031229\\
3.92499999999752	1.37177545841883\\
3.94999999999746	1.34815699692761\\
3.97499999999741	1.32453878539479\\
3.99999999999735	1.30092143451854\\
4.02499999999729	1.27730553444717\\
4.04999999999723	1.25369155142056\\
4.07499999999717	1.23007987240371\\
4.09999999999711	1.20647076447611\\
4.12499999999706	1.18286440282633\\
4.149999999997	1.15926085842286\\
4.17499999999694	1.13566022809118\\
4.19999999999688	1.11206196886706\\
4.22499999999682	1.08846563138383\\
4.24999999999676	1.06486831042494\\
4.27499999999671	1.04125838662959\\
4.29999999999665	1.01763363266136\\
4.32499999999659	0.99399358661985\\
4.34999999999653	0.970337834434867\\
4.37499999999647	0.946666007077448\\
4.39999999999641	0.922977778873894\\
4.42499999999636	0.899272863544693\\
4.4499999999963	0.87555101153821\\
4.47499999999624	0.851812008490636\\
4.49999999999618	0.828055673074174\\
4.52499999999612	0.804281856361438\\
4.54999999999607	0.780490437843254\\
4.57499999999601	0.756681323075262\\
4.59999999999595	0.732854443070837\\
4.62499999999589	0.709009753948023\\
4.64999999999583	0.685147234851193\\
4.67499999999577	0.6612668831109\\
4.69999999999572	0.637368714943482\\
4.72499999999566	0.613452750526019\\
4.7499999999956	0.589519036620418\\
4.77499999999554	0.565567643364509\\
4.79999999999548	0.541598651601102\\
4.82499999999542	0.517612154798549\\
4.84999999999537	0.493608264022253\\
4.87499999999531	0.469587094328109\\
4.89999999999525	0.445548774175815\\
4.92499999999519	0.421493444695465\\
4.94999999999513	0.397421244686733\\
4.97499999999507	0.37333233482899\\
4.99999999999502	0.349226864411995\\
5.02499999999496	0.32510500808088\\
5.0499999999949	0.300966919923937\\
5.07499999999484	0.276812943619597\\
5.09999999999478	0.25264340785658\\
5.12499999999473	0.22845844839684\\
5.14999999999467	0.204258205569069\\
5.17499999999461	0.180042823462768\\
5.19999999999455	0.155812448757799\\
5.22499999999449	0.131567229304726\\
5.24999999999443	0.107307312254039\\
5.27499999999438	0.0830328413173943\\
5.29999999999432	0.0587439521733252\\
5.32499999999426	0.0344407631283792\\
5.3499999999942	0.010424819802326\\
};
\addlegendentry{(pure-pursuit,$\theta_A^*$)}
\end{axis}
\end{tikzpicture}%

==> fig/example3/dAD.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.9290, 0.6940, 0.1250}%
\definecolor{mycolor3}{rgb}{0.20000,0.30000,0.70000}%
\definecolor{mycolor4}{rgb}{0.86000,0.08000,0.24000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=6.5cm,
height=3.566cm,
at={(0,0)},
scale only axis,
xlabel style={font=\color{white!15!black}},
xlabel={$t$},
xmin=0,
xmax=0.9,
ymin=0,
ymax=0.4,
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black, font=\tiny}
]
\addplot [color=mycolor2]
  table[row sep=crcr]{%
0.0250000000000002	0.360172650197894\\
0.0500000000000009	0.359037835692116\\
0.0749999999999999	0.357169259251553\\
0.0999999999999971	0.354585037447642\\
0.124999999999994	0.351302839690442\\
0.149999999999992	0.347339899135611\\
0.174999999999989	0.342713023482984\\
0.199999999999986	0.337438605219178\\
0.224999999999983	0.331532632208623\\
0.249999999999981	0.325010697627457\\
0.274999999999978	0.317888009633139\\
0.299999999999975	0.31017940088991\\
0.324999999999972	0.301899337921355\\
0.34999999999997	0.293061929950927\\
0.374999999999967	0.283680937861717\\
0.399999999999964	0.273769782619891\\
0.424999999999961	0.263341554061738\\
0.449999999999959	0.252409018649257\\
0.474999999999956	0.240984627811468\\
0.499999999999953	0.229080525638843\\
0.52499999999995	0.216708556406001\\
0.549999999999948	0.203880271520546\\
0.574999999999945	0.190606937448903\\
0.599999999999942	0.17689954254209\\
0.624999999999939	0.162768803833695\\
0.649999999999937	0.1482251739407\\
0.674999999999934	0.133278847066355\\
0.699999999999931	0.117939766655251\\
0.724999999999928	0.102217632191975\\
0.749999999999926	0.0861218989050279\\
0.774999999999923	0.0696617965692508\\
0.79999999999992	0.052846293910523\\
0.824999999999917	0.0356840994560171\\
0.849999999999915	0.018183986250278\\
0.874099999999912	0.000992472164329625\\
};
\addlegendentry{($\theta_D^*$,$\theta_A^*$)}
\addplot [color=mycolor3]
  table[row sep=crcr]{%
0.0250000000000002	0.360114537540166\\
0.0500000000000009	0.358807916287546\\
0.0749999999999999	0.356657665404137\\
0.0999999999999971	0.35368577222091\\
0.124999999999994	0.349913830055088\\
0.149999999999992	0.345363059943596\\
0.174999999999989	0.340054334059474\\
0.199999999999986	0.334008200476316\\
0.224999999999983	0.32724490992909\\
0.249999999999981	0.319784444437421\\
0.274999999999978	0.311646547804691\\
0.299999999999975	0.302850758879193\\
0.324999999999972	0.293416446180317\\
0.34999999999997	0.283362846630633\\
0.374999999999967	0.272709107534342\\
0.399999999999964	0.261474332286915\\
0.424999999999961	0.249677631198941\\
0.449999999999959	0.237338178343582\\
0.474999999999956	0.224475275734798\\
0.499999999999953	0.211108428181293\\
0.52499999999995	0.197257429811906\\
0.549999999999948	0.182942467956797\\
0.574999999999945	0.168184249187385\\
0.599999999999942	0.153004158426633\\
0.624999999999939	0.137424462619042\\
0.649999999999937	0.121468577057252\\
0.674999999999934	0.105161441834417\\
0.699999999999931	0.0885300496111692\\
0.724999999999928	0.0716042529527261\\
0.749999999999926	0.0544181223044421\\
0.774999999999923	0.0370122729485614\\
0.79999999999992	0.0194379565757712\\
0.824999999999917	0.00178041644803375\\
0.826149999999917	0.000967816880259708\\
};
\addlegendentry{($\theta_D^*$,pure-pursuit)}
\addplot [color=mycolor4]
  table[row sep=crcr]{%
0.0250000000000002	0.360120365358242\\
0.0500000000000009	0.358829482447499\\
0.0749999999999999	0.356703385833436\\
0.0999999999999971	0.353763969421496\\
0.124999999999994	0.350034043352157\\
0.149999999999992	0.345537298878597\\
0.174999999999989	0.340298299262195\\
0.199999999999986	0.334342506272142\\
0.224999999999983	0.327696342686573\\
0.249999999999981	0.320387282432407\\
0.274999999999978	0.312443978937976\\
0.299999999999975	0.303896460182105\\
0.324999999999972	0.294776368059722\\
0.34999999999997	0.285117335420963\\
0.374999999999967	0.274955617595088\\
0.399999999999964	0.264331266706218\\
0.424999999999961	0.253290703000511\\
0.449999999999959	0.241892019682691\\
0.474999999999956	0.23021424430739\\
0.499999999999953	0.218368117837426\\
0.52499999999995	0.206501970217953\\
0.549999999999948	0.194799724069271\\
0.574999999999945	0.183474265077047\\
0.599999999999942	0.172752455118282\\
0.624999999999939	0.162872294445054\\
0.649999999999937	0.154079321468507\\
0.674999999999934	0.146610802640886\\
0.699999999999931	0.140678296157412\\
0.724999999999928	0.136435192893512\\
0.749999999999926	0.133944183878372\\
0.774999999999923	0.133156201515509\\
0.79999999999992	0.133910627126225\\
0.824999999999917	0.135957940682299\\
0.849999999999915	0.138996113323495\\
0.874999999999912	0.142708042074489\\
0.899999999999909	0.146790630797572\\
0.924999999999906	0.150972283155767\\
0.949999999999904	0.155020261316357\\
0.974999999999901	0.158741300610415\\
0.999999999999898	0.16197843707234\\
1.02499999999995	0.164606269486193\\
1.05	0.166526019756583\\
1.07500000000006	0.167660924389337\\
1.10000000000011	0.167952316071301\\
1.12500000000016	0.167356367246907\\
1.15000000000021	0.165841450392139\\
1.17500000000027	0.163386159671055\\
1.20000000000032	0.159978163712522\\
1.22500000000037	0.155612987543687\\
1.25000000000043	0.150290795360267\\
1.27500000000048	0.144017424798986\\
1.30000000000053	0.136804781559215\\
1.32500000000058	0.128670105519757\\
1.35000000000064	0.119223349247169\\
1.35595000000065	0.116735755971863\\
};
\addlegendentry{(pure-pursuit,$\theta_A^*$)}
\end{axis}
\end{tikzpicture}%

==> fig/example3/dtarget.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.9290, 0.6940, 0.1250}%
\definecolor{mycolor3}{rgb}{0.20000,0.30000,0.70000}%
\definecolor{mycolor4}{rgb}{0.86000,0.08000,0.24000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=6.5cm,
height=3.566cm,
at={(0,0)},
scale only axis,
xlabel style={font=\color{white!15!black}},
xlabel={$t$},
xmin=0,
xmax=0.9,
ymin=0.3,
ymax=0.65,
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black,font=\tiny}
]
\addplot [color=mycolor2]
  table[row sep=crcr]{%
0.0250000000000002	0.607973718169301\\
0.0500000000000009	0.607076137671274\\
0.0749999999999999	0.605598332235999\\
0.0999999999999971	0.603554838862538\\
0.124999999999994	0.600959916209772\\
0.149999999999992	0.597827550913682\\
0.174999999999989	0.594171464959653\\
0.199999999999986	0.590005123868651\\
0.224999999999983	0.585341746041666\\
0.249999999999981	0.580194312855049\\
0.274999999999978	0.574575579696315\\
0.299999999999975	0.568498088051814\\
0.324999999999972	0.561974178726373\\
0.34999999999997	0.555016006175848\\
0.374999999999967	0.547635554385643\\
0.399999999999964	0.539844654220186\\
0.424999999999961	0.53165500290346\\
0.449999999999959	0.523078185330182\\
0.474999999999956	0.51412569833399\\
0.499999999999953	0.504808977853198\\
0.52499999999995	0.495139429807221\\
0.549999999999948	0.485128465237806\\
0.574999999999945	0.47478754142002\\
0.599999999999942	0.464128209095117\\
0.624999999999939	0.453162167791282\\
0.649999999999937	0.441901331143455\\
0.674999999999934	0.430357903940964\\
0.699999999999931	0.418544475302791\\
0.724999999999928	0.40647413041796\\
0.749999999999926	0.394160581563335\\
0.774999999999923	0.381618340695107\\
0.79999999999992	0.368862895439295\\
0.824999999999917	0.355910953579788\\
0.849999999999915	0.34278098394864\\
0.874099999999912	0.329977769186367\\
};
\addlegendentry{($\theta_D^*$,$\theta_A^*$)}
\addplot [color=mycolor3]
  table[row sep=crcr]{%
0.0250000000000002	0.607966341001509\\
0.0500000000000009	0.607046828529146\\
0.0749999999999999	0.605532766701325\\
0.0999999999999971	0.603438834993935\\
0.124999999999994	0.600779350445317\\
0.149999999999992	0.597568276604869\\
0.174999999999989	0.593819232260734\\
0.199999999999986	0.589545499951974\\
0.224999999999983	0.584760034270593\\
0.249999999999981	0.579475469958578\\
0.274999999999978	0.573704129805027\\
0.299999999999975	0.567458032348289\\
0.324999999999972	0.560748899387947\\
0.34999999999997	0.553588163311315\\
0.374999999999967	0.545986974239066\\
0.399999999999964	0.537956206994406\\
0.424999999999961	0.529506467900206\\
0.449999999999959	0.520648101408286\\
0.474999999999956	0.511391196565045\\
0.499999999999953	0.501745593317436\\
0.52499999999995	0.491720888663259\\
0.549999999999948	0.481326442649591\\
0.574999999999945	0.470571384223125\\
0.599999999999942	0.459464616936057\\
0.624999999999939	0.448014824511094\\
0.649999999999937	0.436230476269069\\
0.674999999999934	0.424119832422536\\
0.699999999999931	0.411690949238676\\
0.724999999999928	0.398951684074722\\
0.749999999999926	0.385909700289069\\
0.774999999999923	0.372572472031117\\
0.79999999999992	0.358947288912861\\
0.824999999999917	0.345041260565134\\
0.826149999999917	0.344394941134631\\
};
\addlegendentry{($\theta_D^*$,pure-pursuit)}
\addplot [color=mycolor4]
  table[row sep=crcr]{%
0.0250000000000002	0.607973595485824\\
0.0500000000000009	0.60707513208476\\
0.0749999999999999	0.605594855115603\\
0.0999999999999971	0.603546388094269\\
0.124999999999994	0.600942978144671\\
0.149999999999992	0.597797489675663\\
0.174999999999989	0.59412239856291\\
0.199999999999986	0.589929790428543\\
0.224999999999983	0.585231365651957\\
0.249999999999981	0.580038453268802\\
0.274999999999978	0.574362043002163\\
0.299999999999975	0.568212850936097\\
0.324999999999972	0.561601434196706\\
0.34999999999997	0.554538393505939\\
0.374999999999967	0.547034701634713\\
0.399999999999964	0.539102177506435\\
0.424999999999961	0.5307539734829\\
0.449999999999959	0.522004558658573\\
0.474999999999956	0.51286828846485\\
0.499999999999953	0.503356718276039\\
0.52499999999995	0.493477093550357\\
0.549999999999948	0.483233671552903\\
0.574999999999945	0.472630368179363\\
0.599999999999942	0.461676964087178\\
0.624999999999939	0.450381205599074\\
0.649999999999937	0.438747243848206\\
0.674999999999934	0.426783419075248\\
0.699999999999931	0.414497866377081\\
0.724999999999928	0.401898520655127\\
0.749999999999926	0.388993121506191\\
0.774999999999923	0.375789218055271\\
0.79999999999992	0.362294173531746\\
0.824999999999917	0.348515169844384\\
0.849999999999915	0.334459212078745\\
0.874999999999912	0.320133132701123\\
0.899999999999909	0.305543595948393\\
0.924999999999906	0.290697101775671\\
0.949999999999904	0.275599989383057\\
0.974999999999901	0.260258442141508\\
0.999999999999898	0.244678491282954\\
1.02499999999995	0.228866019217937\\
1.05	0.212826763536158\\
1.07500000000006	0.196566320150969\\
1.10000000000011	0.180090147112988\\
1.12500000000016	0.163403568058368\\
1.15000000000021	0.146511775407866\\
1.17500000000027	0.129419834820268\\
1.20000000000032	0.112132694032287\\
1.22500000000037	0.09465518436276\\
1.25000000000043	0.0769919932874934\\
1.27500000000048	0.0591476900112553\\
1.30000000000053	0.0411267338501871\\
1.32500000000058	0.0229345618228529\\
1.35000000000064	0.00502490731050115\\
1.35595000000065	0.000976312925175253\\
};
\addlegendentry{(pure-pursuit,$\theta_A^*$)}
\end{axis}
\end{tikzpicture}%

==> not-used-part.tex <==
\begin{theorem}\label{thm:part-opti}
    On $\mathcal{L}$, if the minimal point to the target satisfies that $\sin(\theta_A-\phi),\sin(\theta_D-\phi),\sin(\theta_A-\theta_D) $ have the same sign, strategy I satisfies $H=0$. 
\end{theorem}
\begin{proof}

We first reformulate the Hamiltonian in \eqref{eq:Hamiltonian1}. 
Substituting \eqref{eq:optimal_condition} into \eqref{eq:costate}, the co-states can be rewritten as:
\begin{equation}
\label{eq:co-states}
    \begin{aligned}
        \lambda_1 &= \left|\nu\right|\cos\theta_D,\lambda_2=\left|\nu\right|\sin\theta_D,\\
        \gamma_1 &= -\left|\gamma\right|\cos\theta_A,\gamma_2=-\left|\gamma\right|\sin\theta_A.\\
    \end{aligned}
\end{equation}
where $\left|\gamma\right|=\sqrt{\gamma_1^2+\gamma_2^2},\ \left|\nu\right|>0$. By combining \eqref{eq:co-states} and \eqref{eq:costate}, we have the value of $|\nu|$ in terms of $\theta_i$ and $\phi$:
\begin{equation}\label{eq:nu}
    \begin{aligned}
        &\frac{\gamma_2}{\gamma_1}=\frac{\sin\phi-|\nu|\sin\theta_D}{\cos\phi-|\nu|\cos\theta_D}=\tan\theta_A\\
        \Rightarrow &\left|\nu\right|=\frac{\sin(\theta_A-\phi)}{\sin(\theta_A-\theta_D)},
    \end{aligned}
\end{equation}
where $\cos\phi=\frac{x_{Af}}{\sqrt{x_{Af}^2+y_{Af}^2}},\sin\phi=\frac{y_{Af}}{\sqrt{x_{Af}^2+y_{Af}^2}}$. Then, $|\gamma|$ can be formulated as follows:
\begin{equation}
\label{eq:gamma}
    \begin{aligned}
        \left|\gamma\right|&=\sqrt{1+\nu^2-2\left|\nu\right|\cos(\phi-\theta_D)}\\
        &=\sqrt{
        \begin{aligned}
            1+&(\frac{S_\phi C_A-C_\phi S_A}{S_AC_D-C_AS_D})^2\\
            &+2\frac{S_\phi C_A-C_\phi S_A}{S_AC_D-C_AS_D}(C_\phi C_D+S_\phi S_D)
            % 1+&(\frac{S_\phi C_A-C_\phi S_A}{S_AC_D-C_AS_D})^2+2\frac{S_\phi C_A-C_\phi S_A}{S_AC_D-C_AS_D}(C_\phi C_D+S_\phi S_D)
        \end{aligned}
        }\\
        &=\left|\frac{\sin(\theta_D-\phi)}{\sin(\theta_A-\theta_D)}\right|,
    \end{aligned}
\end{equation}
where $S$ is the abbreviation of $\sin$, and $C$ the abbreviation of $\cos$.

Combining \eqref{eq:Hamiltonian1}, \eqref{eq:motion}, \eqref{eq:co-states}, \eqref{eq:nu} and \eqref{eq:gamma}, the Hamiltonian at the terminal time can be formulated as:
\begin{equation}
\label{eq:Hamiltonian2}
\begin{aligned}
    H\ =\ &\left|\nu\right|(v_{Dx0}\cos\theta_D+v_{Dy0}\sin\theta_D)e^{-\mu t_f}\\
    -&\left|\gamma\right|(v_{Ax0}\cos\theta_A+v_{Ay0}\sin\theta_A)e^{-\mu t_f}\\
    +&\left|\nu\right|\frac{u_{Dm}}{\mu}(1-e^{-\mu t_f})-\left|\gamma\right|\frac{u_{Am}}{\mu}(1-e^{-\mu t_f})\\
    =\ &\left|\nu\right|(v_{Dxf}\cos\theta_D+v_{Dyf}\sin\theta_D)\\
    -&\left|\gamma\right|(v_{Axf}\cos\theta_A+v_{Ayf}\sin\theta_A)\\
    =\ &\frac{\sin(\theta_A-\phi)}{\sin(\theta_A-\theta_D)}(v_{Dxf}\cos\theta_D+v_{Dyf}\sin\theta_D)\\
    -&\left|\frac{\sin(\theta_D-\phi)}{\sin(\theta_A-\theta_D)}\right|(v_{Axf}\cos\theta_A+v_{Ayf}\sin\theta_A).
\end{aligned}
% \begin{aligned}
%     H=\ &\left|\nu\right|(v_{Dxf}\cos\theta_D+v_{Dyf}\sin\theta_D)-\left|\gamma\right|(v_{Axf}\cos\theta_A+v_{Ayf}\sin\theta_A)\\
%     =\ &\frac{\sin(\theta_A-\phi)}{\sin(\theta_A-\theta_D)}(v_{Dxf}\cos\theta_D+v_{Dyf}\sin\theta_D)-\left|\frac{\sin(\theta_D-\phi)}{\sin(\theta_A-\theta_D)}\right|(v_{Axf}\cos\theta_A+v_{Ayf}\sin\theta_A).
% \end{aligned}
\end{equation}
% We should note here that the form in \eqref{eq:Hamiltonian2} is derived under the assumption that the attacker and the defender adopt strategies satisfying \eqref{eq:optimal_condition}.


Let points on $\mathcal{L}$ be $[x_f(t),y_f(t)]^T$, where $t$ is the time that isochrones intersect at the points. The local minimal point of the payoff function satisfies:
\begin{equation}\label{eq:minimal-condition}
    x_f\frac{d x_f}{dt}+y_f\frac{d y_f}{dt}=0.
\end{equation}
We first calculate $\frac{dx_f}{dt}$ and $\frac{dy_f}{dt} $:
\begin{equation}\label{eq:d_xf}
\begin{aligned}
    \frac{dx_f}{dt} = \frac{dx_{Af}}{dt}=\frac{dx_{Df}}{dt},\\
    \frac{dy_f}{dt} = \frac{dy_{Af}}{dt}=\frac{dy_{Df}}{dt}. 
\end{aligned}  
\end{equation}
By regarding $\theta_i$ as a function of $t$, we have:
\begin{equation}\label{eq:dxdt}
\begin{aligned}
    \frac{dx_{if}}{dt}&=\frac{\partial x_{if}}{\partial t}+\frac{\partial x_{if}}{\partial\theta_i}\frac{d\theta_i}{dt},\\
    \frac{dy_{if}}{dt}&=\frac{\partial y_{if}}{\partial t}+\frac{\partial y_{if}}{\partial\theta_i}\frac{d\theta_i}{dt},\\
\end{aligned}
\end{equation}
where
\begin{equation}
    \begin{aligned}
    \frac{\partial x_i}{\partial \theta_i} &= -\frac{u_i\sin\theta_i}{\mu}(t-\frac{1-e^{-\mu t}}{\mu}),\\
    \frac{\partial y_i}{\partial \theta_i} &= \frac{u_i\cos\theta_i}{\mu}(t-\frac{1-e^{-\mu t}}{\mu}),
    \end{aligned}
\end{equation}
is derived from \eqref{eq:motion}.
Equation \eqref{eq:d_xf} can be rewritten as:
\begin{equation}
    \begin{bmatrix}
    \frac{\partial x_{Af}}{\partial\theta_A}&-\frac{\partial x_{Df}}{\partial\theta_D}\\
    \frac{\partial y_{Af}}{\partial\theta_A}&-\frac{\partial y_{Df}}{\partial\theta_D}\\
    \end{bmatrix}
    \begin{bmatrix}
        \frac{d\theta_A}{dt}\\\frac{d\theta_D}{dt}
    \end{bmatrix}=
    \begin{bmatrix}
        \frac{\partial x_{Df}}{\partial t}-\frac{\partial x_{Af}}{\partial t}\\
        \frac{\partial y_{Df}}{\partial t}-\frac{\partial y_{Af}}{\partial t}
    \end{bmatrix}.
\end{equation}
By solving this equation we get:
$$\frac{d\theta_A}{dt}=\frac{\frac{\partial y_{Df}}{\partial \theta_D}\frac{\partial x_{Af}}{\partial t}-\frac{\partial y_{Df}}{\partial \theta_D}\frac{\partial x_{Df}}{\partial t}+\frac{\partial x_{Df}}{\partial \theta_D}\frac{\partial y_{Df}}{\partial t}-\frac{\partial x_{Df}}{\partial \theta_D}\frac{\partial y_{Af}}{\partial t}}{\frac{\partial y_{Af}}{\partial \theta_A}\frac{\partial x_{Df}}{\partial \theta_D}-\frac{\partial x_{Af}}{\partial \theta_A}\frac{\partial y_{Df}}{\partial \theta_D}},$$
Substituting this into \eqref{eq:dxdt} we get:
\begin{equation}
    \begin{aligned}
        \frac{dx_f}{dt}=&
        \begin{aligned}
            \left(\begin{aligned}
            &e^{-\mu t}(v_{Dx0}\cos\theta_D+v_{Dy0}\sin\theta_D)\sin\theta_A\\
            -&e^{-\mu t}(v_{Ax0}\cos\theta_A+v_{Ay0}\sin\theta_A)\sin\theta_D\\
            +&(1-e^{-\mu t})\frac{u_D\sin\theta_A-u_A\sin\theta_D}{\mu} 
            \end{aligned}
            \right)&\\
            /\sin(\theta_A-\theta_D)&
        \end{aligned}
        \\
        =&\frac{\left(\splitdfrac{(v_{Dxf}\cos\theta_D+v_{Dyf}\sin\theta_D)\sin\theta_A}{-(v_{Axf}\cos\theta_A+v_{Ayf}\sin\theta_A)\sin\theta_D}\right)}{\sin(\theta_A-\theta_D)}.\\
        \end{aligned}
\end{equation} 
Similarly we can get:
\begin{equation}
    \begin{aligned}
        \frac{dy_f}{dt}=&\frac{\left(\splitdfrac{(v_{Axf}\cos\theta_A+v_{Ayf}\sin\theta_A)\cos\theta_D}{-(v_{Dxf}\cos\theta_D+v_{Dyf}\sin\theta_D)\cos\theta_A}\right)}{\sin(\theta_A-\theta_D)}.
    \end{aligned}
\end{equation}
Based on this, \eqref{eq:minimal-condition} can be rewritten as:
\begin{equation}
    \begin{aligned}
        \frac{\left(\splitdfrac{(x_f\sin\theta_A-y_f\cos\theta_A)(v_{Dxf}\cos\theta_D+v_{Dyf}\sin\theta_D)}
        {-(x_f\sin\theta_D-y_f\cos\theta_D)(v_{Axf}\cos\theta_A+v_{Ayf}\sin\theta_A)}\right)}{\sin(\theta_A-\theta_D)}&\\=0&\\
        \Longrightarrow\frac{\left(\splitdfrac{\sin(\theta_A-\phi)(v_{Dxf}\cos\theta_D+v_{Dyf}\sin\theta_D)}{-\sin(\theta_D-\phi)(v_{Axf}\cos\theta_A+v_{Ayf}\sin\theta_A)}\right)}{\sin(\theta_A-\theta_D)}=0&.
    \end{aligned}
\end{equation}
Comparing this with \eqref{eq:Hamiltonian2}, we can see that if $\sin(\theta_A-\phi),\sin(\theta_D-\phi)$ have the same sign at the terminal point, and the point is the local minimal point, $H=0$ is satisfied. Moreover, \eqref{eq:nu} requires that $\sin(\theta_A-\theta_D)$ and $\sin(\theta_A-\phi)$ to have the same sign.

\end{proof}

\begin{figure}
    \centering
    \input{fig/angle}
    \caption{geometric illustration of the constraint in Theorem \ref{thm:part-opti}. $\mathbf{x}_{Dc}$ and $\mathbf{x}_{Ac}$ represent the centers of isochrones at terminal time $t_f$. $\mathbf{x}_f$ represents the intersection of isochrones.}
    \label{fig:geometric-condition}
\end{figure}

A geometric illustration for the constraint is given in Fig.\ref{fig:geometric-condition}. If $\mathbf{x}_f \in \Omega_I\cup\Omega_{II}$, $\frac{\sin(\theta_A-\phi)}{\sin(\theta_A-\theta_D)}>0$ is satisfied. If $\mathbf{x}_f \in \Omega_I\cup\Omega_{III}$, $\frac{\sin(\theta_D-\phi)}{\sin(\theta_A-\theta_D)}>0$ is satisfied. $H=0$ holds only if $\mathbf{x}_f\in\Omega_I$. 
